Pegasus-v1 Technical Report

This technical report introduces Pegasus-1, a multimodal language model specialized in video content understanding and interaction through natural language. Pegasus-1 is designed to address the unique challenges posed by video data, such as interpreting spatiotemporal information, to offer nuanced video content comprehension across various lengths. This technical report overviews Pegasus-1's architecture, training strategies, and its performance in benchmarks on video conversation, zero-shot video question answering, and video summarization. We also explore qualitative characteristics of Pegasus-1 , demonstrating its capabilities as well as its limitations, in order to provide readers a balanced view of its current state and its future direction.

==> tables/tempcompass.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}ccccccccccccc@{}}
% \toprule
% \multicolumn{1}{l}{} & \multicolumn{2}{c}{Action} & \multicolumn{2}{c}{Direction} & \multicolumn{2}{c}{Speed} & \multicolumn{1}{l}{Event Order} & \multicolumn{4}{c}{Attribute Change} & \multicolumn{1}{l}{} \\ \midrule
% \textbf{}            & fine        & coarse       & object        & camera        & absolute    & relative    & order                           & color   & size  & combined  & other  & Avg.                 \\
% Human                & \multicolumn{2}{c}{99.3}   & \multicolumn{2}{c}{91.2}      & \multicolumn{2}{c}{96.1}  & 98.6                            & \multicolumn{4}{c}{100.0}            &                      \\
% Random               & 37.2        & 37.7         & 37.3          & 36.2          & 38.6        & 40.0        & 39.5                            & 38.1    & 37.5  & 36.1      & 36.6   & 38.1                 \\
% mPLUG-Owl            & 48.2        & 67.0         & 36.1          & 34.6          & 40.3        & 36.0        & 40.1                            & 38.8    & 42.9  & 40.3      & 41.6   & 42.7                 \\
% V-LLaVA              & 54.6        & 82.6         & 39.6          & 39.9          & 44.1        & 39.7        & 45.3                            & 44.3    & 44.5  & 41.4      & 50.9   & 48.3                 \\
% VideoChat2           & 62.4        & 78.8         & 43.4          & 37.5          & 52.0        & 39.5        & 43.5                            & 50.9    & 46.7  & 48.2      & 42.4   & 50.0                 \\
% Pegasus              & 81.6        & 93.4         & 44.4          & 42.4          & 47.9        & 42.2        & 55.8                            & 51.8    & 49.8  & 45.7      & 43.9   & 56.5                 \\ \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[]
\centering
\tiny
\begin{adjustbox}{center}
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Action}} & \multicolumn{2}{c|}{\textbf{Direction}} & \multicolumn{2}{c|}{\textbf{Speed}}   & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Event\\ Order\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attribute\\ Change\end{tabular}}} & \multicolumn{1}{l}{\textbf{}} \\ \midrule
                      & \textbf{Fine}     & \textbf{Coarse}  & \textbf{Object}    & \textbf{Camera}    & \textbf{Absolute} & \textbf{Relative} & \textbf{Order}                                                                      & \textbf{Color}       & \textbf{Size}       & \textbf{Combined}     & \textbf{Other}      & \textbf{Avg.}                 \\
Human                 & \multicolumn{2}{c|}{99.3\%}          & \multicolumn{2}{c|}{91.2\%}             & \multicolumn{2}{c|}{96.1\%}           & 98.6\%                                                                              & \multicolumn{4}{c|}{100.0\%}                                                             &                               \\
Random                & 37.2\%            & 37.7\%           & 37.3\%             & 36.2\%             & 38.6\%            & 40.0\%            & 39.5\%                                                                              & 38.1\%               & 37.5\%              & 36.1\%                & 36.6\%              & 38.1\%                        \\
mPLUG-Owl             & 48.2\%            & 67.0\%           & 36.1\%             & 34.6\%             & 40.3\%            & 36.0\%            & 40.1\%                                                                              & 38.8\%               & 42.9\%              & 40.3\%                & 41.6\%              & 42.7\%                        \\
V-LLaVA               & 54.6\%            & 82.6\%           & 39.6\%             & 39.9\%             & 44.1\%            & 39.7\%            & 45.3\%                                                                              & 44.3\%               & 44.5\%              & 41.4\%                & 50.9\%              & 48.3\%                        \\
VideoChat2            & 62.4\%            & 78.8\%           & 43.4\%             & 37.5\%             & 52.0\%            & 39.5\%            & 43.5\%                                                                              & 50.9\%               & 46.7\%              & 48.2\%                & 42.4\%              & 50.0\%                        \\ \midrule
Pegasus               & \textbf{81.6\%}   & \textbf{93.4\%}  & \textbf{44.4\%}    & \textbf{42.4\%}    & \textbf{47.9\%}   & \textbf{42.2\%}   & \textbf{55.8\%}                                                                     & \textbf{51.8\%}      & \textbf{49.8\%}     & \textbf{45.7\%}       & \textbf{43.9\%}     & \textbf{56.5\%}      \\  \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{5pt}
\caption{Result on TempCompass~\cite{liu2024tempcompass}}
\label{tab:tempcompass}
\end{table}

==> tables/tempcompass2.tex <==
% \begin{table}[]
% \begin{tabular}{@{}c|cc|cc|cc|c|cccc|c@{}}
% \toprule
% \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Action}} & \multicolumn{2}{c|}{\textbf{Direction}} & \multicolumn{2}{c|}{\textbf{Speed}}   & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Event\\ Order\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attribute\\ Change\end{tabular}}} & \multicolumn{1}{l}{\textbf{}} \\ \midrule
%                       & \textbf{Fine}     & \textbf{Coarse}  & \textbf{Object}    & \textbf{Camera}    & \textbf{Absolute} & \textbf{Relative} & \textbf{Order}                                                                      & \textbf{Color}       & \textbf{Size}       & \textbf{Combined}     & \textbf{Other}      & \textbf{Avg.}                 \\
% Human                 & \multicolumn{2}{c|}{99.3\%}          & \multicolumn{2}{c|}{91.2\%}             & \multicolumn{2}{c|}{96.1\%}           & 98.6\%                                                                              & \multicolumn{4}{c|}{100.0\%}                                                             &                               \\
% Random                & 37.2\%            & 37.7\%           & 37.3\%             & 36.2\%             & 38.6\%            & 40.0\%            & 39.5\%                                                                              & 38.1\%               & 37.5\%              & 36.1\%                & 36.6\%              & 38.1\%                        \\
% mPLUG-Owl             & 48.2\%            & 67.0\%           & 36.1\%             & 34.6\%             & 40.3\%            & 36.0\%            & 40.1\%                                                                              & 38.8\%               & 42.9\%              & 40.3\%                & 41.6\%              & 42.7\%                        \\
% V-LLaVA               & 54.6\%            & 82.6\%           & 39.6\%             & 39.9\%             & 44.1\%            & 39.7\%            & 45.3\%                                                                              & 44.3\%               & 44.5\%              & 41.4\%                & 50.9\%              & 48.3\%                        \\
% VideoChat2            & 62.4\%            & 78.8\%           & 43.4\%             & 37.5\%             & 52.0\%            & 39.5\%            & 43.5\%                                                                              & 50.9\%               & 46.7\%              & 48.2\%                & 42.4\%              & 50.0\%                        \\ \midrule
% Pegasus               & \textbf{81.6\%}   & \textbf{93.4\%}  & \textbf{44.4\%}    & \textbf{42.4\%}    & \textbf{47.9\%}   & \textbf{42.2\%}   & \textbf{55.8\%}                                                                     & \textbf{51.8\%}      & \textbf{49.8\%}     & \textbf{45.7\%}       & \textbf{43.9\%}     & \textbf{56.5\%}              
% \end{tabular}
% \end{table}


\begin{table}[htbp]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|cc|cc|cc|c|cccc|c@{}}
\hline
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{Action}} & \multicolumn{2}{c|}{\textbf{Direction}} & \multicolumn{2}{c|}{\textbf{Speed}}   & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Event\\ Order\end{tabular}}} & \multicolumn{4}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Attribute\\ Change\end{tabular}}} & \multicolumn{1}{l}{\textbf{}} \\ \hline
                      & \textbf{Fine}     & \textbf{Coarse}  & \textbf{Object}    & \textbf{Camera}    & \textbf{Absolute} & \textbf{Relative} & \textbf{Order}                                                                      & \textbf{Color}       & \textbf{Size}       & \textbf{Combined}     & \textbf{Other}      & \textbf{Avg.}                 \\
Human                 & \multicolumn{2}{c|}{99.3\%}          & \multicolumn{2}{c|}{91.2\%}             & \multicolumn{2}{c|}{96.1\%}           & 98.6\%                                                                              & \multicolumn{4}{c|}{100.0\%}                                                             & {97.0\%}                              \\
Random                & 37.2\%            & 37.7\%           & 37.3\%             & 36.2\%             & 38.6\%            & 40.0\%            & 39.5\%                                                                              & 38.1\%               & 37.5\%              & 36.1\%                & 36.6\%              & 38.1\%                        \\
mPLUG-Owl~\cite{DBLP:mplugowl}             & 48.2\%            & 67.0\%           & 36.1\%             & 34.6\%             & 40.3\%            & 36.0\%            & 40.1\%                                                                              & 38.8\%               & 42.9\%              & 40.3\%                & 41.6\%              & 42.7\%                        \\
V-LLaVA~\cite{DBLP:video-llava}               & 54.6\%            & 82.6\%           & 39.6\%             & 39.9\%             & 44.1\%            & 39.7\%            & 45.3\%                                                                              & 44.3\%               & 44.5\%              & 41.4\%                & 50.9\%              & 48.3\%                        \\
VideoChat2~\cite{li2023mvbench}            & 62.4\%            & 78.8\%           & 43.4\%             & 37.5\%             & 52.0\%            & 39.5\%            & 43.5\%                                                                              & 50.9\%               & 46.7\%              & 48.2\%                & 42.4\%              & 50.0\%                        \\ \hline
Pegasus-1               & \textbf{81.6\%}   & \textbf{93.4\%}  & \textbf{44.4\%}    & \textbf{42.4\%}    & \textbf{47.9\%}   & \textbf{42.2\%}   & \textbf{55.8\%}                                                                     & \textbf{51.8\%}      & \textbf{49.8\%}     & \textbf{45.7\%}       & \textbf{43.9\%}     & \textbf{56.5\%}              \\
\hline
\end{tabular}%
}
\vspace{5pt}
\caption{TempCompass~\cite{liu2024tempcompass} assesses the temporal understanding capabilities of video language models across five dimensions. }
\label{tab:tempcompass}
\end{table}
